Breathing K-Means: Superior K-Means Solutions through Dynamic K-Values

We introduce the breathing k-means algorithm, which on average significantly improves solutions obtained by the widely-known greedy k-means++ algorithm, the default method for k-means clustering in the scikit-learn package. The improvements are achieved through a novel ``breathing'' technique, that cyclically increases and decreases the number of centroids based on local error and utility measures. We conducted experiments using greedy k-means++ as a baseline, comparing it with breathing k-means and five other k-means algorithms. Among the methods investigated, only breathing k-means and better k-means++ consistently outperformed the baseline, with breathing k-means demonstrating a substantial lead. This superior performance was maintained even when comparing the best result of ten runs for all other algorithms to a single run of breathing k-means, highlighting its effectiveness and speed. Our findings indicate that the breathing k-means algorithm outperforms the other k-means techniques, especially greedy k-means++ with ten repetitions, which it dominates in both solution quality and speed. This positions breathing k-means (with the built-in initialization by a single run of greedy k-means++) as a superior alternative to running greedy k-means++ on its own.

==> coltables/cpu_one-top.tex <==
\begin{tabular}{lrrrrrrr}
\toprule
problem group & t(\thead{greedy \\ km++}) & \thead{vanilla \\ km++} & \thead{better \\ km++} & \thead{Hartigan- \\ Wong} & \thead{genetic \\ algorithm} & \thead{random \\ swap} & \thead{breathing \\ k-means} \\
\midrule
Known Optimum & {\cellcolor{blue}} \color[HTML]{FFFFFF} 0.69s & {\cellcolor[HTML]{D6EBD6}} \color[HTML]{000000} 83.8\% & {\cellcolor[HTML]{FFDDDD}} \color[HTML]{000000} 754.8\% & {\cellcolor[HTML]{2E972E}} \color[HTML]{FFFFFF} 18.2\% & {\cellcolor[HTML]{FFF6F6}} \color[HTML]{000000} 289.4\% & {\cellcolor[HTML]{FF2323}} \color[HTML]{FFFFFF} 4327.4\% & {\cellcolor[HTML]{61B061}} \color[HTML]{000000} 38.2\% \\
Literature & {\cellcolor{blue}} \color[HTML]{FFFFFF} 0.57s & {\cellcolor[HTML]{D5EAD5}} \color[HTML]{000000} 83.3\% & {\cellcolor[HTML]{FFE7E7}} \color[HTML]{000000} 568.2\% & {\cellcolor[HTML]{219021}} \color[HTML]{FFFFFF} 13.1\% & {\cellcolor[HTML]{FFF8F8}} \color[HTML]{000000} 237.1\% & {\cellcolor[HTML]{FF8585}} \color[HTML]{000000} 2439.9\% & {\cellcolor[HTML]{74BA74}} \color[HTML]{000000} 45.5\% \\
Modified Literature & {\cellcolor{blue}} \color[HTML]{FFFFFF} 0.68s & {\cellcolor[HTML]{ABD5AB}} \color[HTML]{000000} 67.0\% & {\cellcolor[HTML]{FFCBCB}} \color[HTML]{000000} 1104.1\% & {\cellcolor[HTML]{71B871}} \color[HTML]{000000} 44.5\% & {\cellcolor[HTML]{FFE7E7}} \color[HTML]{000000} 575.9\% & {\cellcolor[HTML]{FF0000}} \color[HTML]{FFFFFF} 36358.1\% & {\cellcolor[HTML]{85C285}} \color[HTML]{000000} 52.3\% \\
Evil Spiral & {\cellcolor{blue}} \color[HTML]{FFFFFF} 0.98s & {\cellcolor[HTML]{A9D4A9}} \color[HTML]{000000} 66.1\% & {\cellcolor[HTML]{FFBCBC}} \color[HTML]{000000} 1398.4\% & {\cellcolor[HTML]{43A143}} \color[HTML]{FFFFFF} 26.3\% & {\cellcolor[HTML]{FFEDED}} \color[HTML]{000000} 454.5\% & {\cellcolor[HTML]{FF3B3B}} \color[HTML]{FFFFFF} 3857.2\% & {\cellcolor[HTML]{9ACD9A}} \color[HTML]{000000} 60.5\% \\
High-Dimensional & {\cellcolor{blue}} \color[HTML]{FFFFFF} 0.95s & {\cellcolor[HTML]{DAEDDA}} \color[HTML]{000000} 85.4\% & {\cellcolor[HTML]{FFD6D6}} \color[HTML]{000000} 903.1\% & {\cellcolor[HTML]{FFFBFB}} \color[HTML]{000000} 195.6\% & {\cellcolor[HTML]{FFB3B3}} \color[HTML]{000000} 1571.5\% & {\cellcolor[HTML]{FF0000}} \color[HTML]{FFFFFF} 69674.6\% & {\cellcolor[HTML]{D0E8D0}} \color[HTML]{000000} 81.3\% \\
\midrule
Mean & {\cellcolor{blue}} \color[HTML]{FFFFFF} 0.77s & {\cellcolor[HTML]{C5E2C5}} \color[HTML]{000000} 77.1\% & {\cellcolor[HTML]{FFD3D3}} \color[HTML]{000000} 945.7\% & {\cellcolor[HTML]{98CC98}} \color[HTML]{000000} 59.5\% & {\cellcolor[HTML]{FFE4E4}} \color[HTML]{000000} 625.7\% & {\cellcolor[HTML]{FF0000}} \color[HTML]{FFFFFF} 23331.4\% & {\cellcolor[HTML]{8EC78E}} \color[HTML]{000000} 55.6\% \\
\toprule
\end{tabular}


==> coltables/msestd-espiralX.tex <==
\begin{tabular}{lrrrrrrrrrrrrrrrr}
\toprule
data set & n & k & kmpp1 & kmpp-orig1 & betterkmpp & \thead{Hartigan- \\ Wong} & ga & rs & bkm01 & bkm03 & bkm05 & bkm10 & bkm15 & bkm20 & bkm25 & bkm30 \\
\midrule
espiral01 & 1000.000000 & 100.000000 & 2.4\% & 5.3\% & 1.8\% & 323.1\% & 0.5\% & 0.5\% & 2.2\% & 1.0\% & 0.8\% & 0.7\% & 0.6\% & 0.5\% & 0.4\% & 0.4\% \\
espiral04 & 2500.000000 & 100.000000 & 2.5\% & 5.2\% & 2.1\% & 1271.4\% & 0.7\% & 0.8\% & 1.8\% & 1.1\% & 0.8\% & 0.7\% & 0.5\% & 0.5\% & 0.4\% & 0.4\% \\
espiral07 & 4000.000000 & 100.000000 & 2.1\% & 5.0\% & 1.8\% & 1412.6\% & 3.5\% & 0.9\% & 1.6\% & 1.2\% & 0.9\% & 0.6\% & 0.6\% & 0.5\% & 0.4\% & 0.4\% \\
espiral10 & 5500.000000 & 100.000000 & 2.3\% & 4.7\% & 1.6\% & 1061.5\% & 5.7\% & 1.0\% & 1.8\% & 1.0\% & 0.9\% & 0.6\% & 0.5\% & 0.5\% & 0.4\% & 0.4\% \\
espiral13 & 7000.000000 & 100.000000 & 2.6\% & 4.5\% & 1.5\% & 889.4\% & 12.6\% & 1.1\% & 1.7\% & 1.1\% & 0.8\% & 0.5\% & 0.5\% & 0.4\% & 0.4\% & 0.4\% \\
espiral16 & 8500.000000 & 100.000000 & 2.1\% & 4.1\% & 1.7\% & 477.5\% & 36.8\% & 1.3\% & 1.9\% & 0.8\% & 0.7\% & 0.6\% & 0.5\% & 0.5\% & 0.5\% & 0.4\% \\
espiral19 & 10000.000000 & 100.000000 & 2.4\% & 4.4\% & 2.2\% & 764.4\% & 25.3\% & 1.6\% & 2.2\% & 0.9\% & 0.7\% & 0.6\% & 0.4\% & 0.4\% & 0.3\% & 0.4\% \\
espiral22 & 11500.000000 & 100.000000 & 2.4\% & 4.5\% & 1.8\% & 759.0\% & 32.6\% & 2.0\% & 1.5\% & 0.9\% & 0.6\% & 0.4\% & 0.4\% & 0.4\% & 0.3\% & 0.3\% \\
espiral25 & 13000.000000 & 100.000000 & 2.1\% & 3.8\% & 2.0\% & 497.9\% & 12.8\% & 2.0\% & 1.9\% & 0.8\% & 0.6\% & 0.4\% & 0.4\% & 0.3\% & 0.3\% & 0.3\% \\
\midrule
Mean & nan & nan & 2.3\% & 4.6\% & 1.8\% & 828.5\% & 14.5\% & 1.2\% & 1.8\% & 1.0\% & 0.8\% & 0.6\% & 0.5\% & 0.4\% & 0.4\% & 0.4\% \\
\toprule
\end{tabular}


==> coltables/msestd-fr-mod.tex <==
\begin{tabular}{lrrrrrrrrrrrrrrrr}
\toprule
data set & n & k & kmpp1 & kmpp-orig1 & betterkmpp & \thead{Hartigan- \\ Wong} & ga & rs & bkm01 & bkm03 & bkm05 & bkm10 & bkm15 & bkm20 & bkm25 & bkm30 \\
\midrule
aggregation-$\ast$ & 4200.000000 & 200.000000 & 3.7\% & 20.6\% & 2.9\% & 38726.4\% & 693.1\% & 283.6\% & 2.0\% & 1.8\% & 1.7\% & 1.6\% & 1.4\% & 1.1\% & 0.8\% & 0.8\% \\
compound-$\ast$ & 4200.000000 & 50.000000 & 3.2\% & 6.6\% & 2.8\% & 370.0\% & 26.2\% & 2.9\% & 2.0\% & 1.4\% & 1.2\% & 0.9\% & 0.8\% & 0.6\% & 0.5\% & 0.5\% \\
d31-$\ast$ & 4200.000000 & 100.000000 & 3.6\% & 10.2\% & 3.0\% & 2607.1\% & 40.9\% & 20.1\% & 2.6\% & 1.3\% & 0.8\% & 0.8\% & 0.7\% & 0.7\% & 0.7\% & 0.7\% \\
flame-$\ast$ & 4200.000000 & 80.000000 & 2.9\% & 3.9\% & 2.5\% & 317.3\% & 5.1\% & 4.4\% & 3.1\% & 1.8\% & 1.4\% & 1.3\% & 0.8\% & 0.8\% & 0.8\% & 0.7\% \\
jain-$\ast$ & 4200.000000 & 30.000000 & 3.2\% & 6.7\% & 2.4\% & 338.6\% & 23.0\% & 1.5\% & 2.1\% & 1.4\% & 0.9\% & 0.7\% & 0.6\% & 0.5\% & 0.6\% & 0.6\% \\
pathbased-$\ast$ & 4200.000000 & 50.000000 & 4.1\% & 7.3\% & 3.2\% & 307.2\% & 14.4\% & 3.1\% & 3.2\% & 1.6\% & 1.1\% & 0.7\% & 0.4\% & 0.4\% & 0.4\% & 0.3\% \\
r15-$\ast$ & 4200.000000 & 30.000000 & 3.4\% & 4.9\% & 2.3\% & 1597.3\% & 206.6\% & 1.2\% & 2.2\% & 0.9\% & 0.8\% & 0.5\% & 0.4\% & 0.4\% & 0.4\% & 0.4\% \\
s2-$\ast$ & 4200.000000 & 100.000000 & 3.7\% & 11.2\% & 2.8\% & 5187.6\% & 42.9\% & 18.7\% & 3.0\% & 1.3\% & 1.1\% & 0.9\% & 0.7\% & 0.8\% & 0.7\% & 0.7\% \\
spiral-$\ast$ & 4200.000000 & 80.000000 & 3.6\% & 8.2\% & 3.2\% & 1011.0\% & 26.9\% & 9.2\% & 2.7\% & 2.1\% & 2.2\% & 0.9\% & 0.8\% & 0.9\% & 0.7\% & 0.7\% \\
\midrule
Mean & nan & nan & 3.5\% & 8.9\% & 2.8\% & 5606.9\% & 119.9\% & 38.3\% & 2.5\% & 1.5\% & 1.3\% & 0.9\% & 0.8\% & 0.7\% & 0.6\% & 0.6\% \\
\toprule
\end{tabular}


==> coltables/msestd-fraenti.tex <==
\begin{tabular}{lrrrrrrrrrrrrrrrr}
\toprule
data set & n & k & kmpp1 & kmpp-orig1 & betterkmpp & \thead{Hartigan- \\ Wong} & ga & rs & bkm01 & bkm03 & bkm05 & bkm10 & bkm15 & bkm20 & bkm25 & bkm30 \\
\midrule
aggregation & 788.000000 & 200.000000 & 1.5\% & 2.4\% & 1.2\% & 3.0\% & 0.5\% & 0.4\% & 1.6\% & 1.3\% & 1.1\% & 0.7\% & 0.7\% & 0.6\% & 0.5\% & 0.5\% \\
compound & 399.000000 & 50.000000 & 2.2\% & 3.7\% & 2.1\% & 8.3\% & 0.8\% & 0.7\% & 2.1\% & 1.2\% & 1.2\% & 1.1\% & 0.8\% & 0.8\% & 0.7\% & 0.7\% \\
d31 & 3100.000000 & 100.000000 & 1.3\% & 2.2\% & 1.0\% & 3.8\% & 0.4\% & 0.2\% & 0.8\% & 0.4\% & 0.4\% & 0.2\% & 0.2\% & 0.2\% & 0.2\% & 0.2\% \\
flame & 240.000000 & 80.000000 & 2.6\% & 4.1\% & 2.2\% & 3.1\% & 0.9\% & 0.6\% & 2.9\% & 1.6\% & 1.3\% & 0.8\% & 0.7\% & 0.7\% & 0.8\% & 0.7\% \\
jain & 373.000000 & 30.000000 & 2.3\% & 4.2\% & 2.2\% & 19.4\% & 0.7\% & 0.1\% & 1.5\% & 1.0\% & 0.9\% & 0.4\% & 0.4\% & 0.3\% & 0.3\% & 0.3\% \\
pathbased & 300.000000 & 50.000000 & 2.9\% & 4.6\% & 2.5\% & 10.2\% & 0.8\% & 0.3\% & 2.9\% & 1.8\% & 1.3\% & 1.1\% & 0.7\% & 0.7\% & 0.7\% & 0.6\% \\
r15 & 600.000000 & 30.000000 & 2.4\% & 2.8\% & 1.8\% & 4.4\% & 0.5\% & 0.2\% & 1.1\% & 0.4\% & 0.4\% & 0.3\% & 0.2\% & 0.3\% & 0.2\% & 0.2\% \\
s2 & 5000.000000 & 100.000000 & 1.0\% & 1.7\% & 0.9\% & 3.8\% & 0.4\% & 0.3\% & 0.8\% & 0.5\% & 0.5\% & 0.4\% & 0.2\% & 0.3\% & 0.2\% & 0.2\% \\
spiral & 312.000000 & 80.000000 & 2.4\% & 5.4\% & 2.1\% & 15.3\% & 0.8\% & 0.5\% & 1.2\% & 1.2\% & 1.1\% & 1.1\% & 1.0\% & 0.9\% & 0.8\% & 0.9\% \\
\midrule
Mean & nan & nan & 2.1\% & 3.5\% & 1.8\% & 7.9\% & 0.6\% & 0.4\% & 1.7\% & 1.1\% & 0.9\% & 0.7\% & 0.6\% & 0.5\% & 0.5\% & 0.5\% \\
\toprule
\end{tabular}


==> coltables/msestd-high-D.tex <==
\begin{tabular}{lrrrrrrrrrrrrrrrr}
\toprule
data set & n & k & kmpp1 & kmpp-orig1 & betterkmpp & \thead{Hartigan- \\ Wong} & ga & rs & bkm01 & bkm03 & bkm05 & bkm10 & bkm15 & bkm20 & bkm25 & bkm30 \\
\midrule
Norm25 & 10000.000000 & 10.000000 & 3.5\% & 5.8\% & 2.1\% & 10.1\% & 0.3\% & 0.4\% & 4.0\% & 2.0\% & 1.7\% & 1.5\% & 1.5\% & 1.6\% & 1.4\% & 1.5\% \\
Norm25 & 10000.000000 & 25.000000 & 0.0\% & 0.0\% & 0.0\% & 83626.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
Norm25 & 10000.000000 & 50.000000 & 0.1\% & 0.2\% & 0.1\% & 42184.7\% & 0.1\% & 0.1\% & 0.1\% & 0.1\% & 0.1\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
Norm25 & 10000.000000 & 100.000000 & 0.1\% & 0.2\% & 0.1\% & 7693.2\% & 0.1\% & 0.1\% & 0.1\% & 0.1\% & 0.1\% & 0.1\% & 0.1\% & 0.1\% & 0.1\% & 0.1\% \\
Norm25 & 10000.000000 & 200.000000 & 0.2\% & 0.2\% & 0.1\% & 0.2\% & 0.1\% & 0.1\% & 0.1\% & 0.1\% & 0.1\% & 0.1\% & 0.1\% & 0.1\% & 0.1\% & 0.1\% \\
Cloud & 1024.000000 & 10.000000 & 5.2\% & 8.5\% & 3.4\% & 1.9\% & 2.9\% & 0.1\% & 2.5\% & 0.5\% & 0.4\% & 0.1\% & 0.1\% & 0.1\% & 0.1\% & 0.1\% \\
Cloud & 1024.000000 & 25.000000 & 2.6\% & 4.5\% & 1.8\% & 24.9\% & 4.3\% & 0.1\% & 1.4\% & 1.0\% & 0.7\% & 0.5\% & 0.4\% & 0.4\% & 0.3\% & 0.2\% \\
Cloud & 1024.000000 & 50.000000 & 1.9\% & 4.0\% & 1.4\% & 9.3\% & 17.0\% & 0.2\% & 1.5\% & 0.6\% & 0.5\% & 0.4\% & 0.3\% & 0.2\% & 0.2\% & 0.2\% \\
Cloud & 1024.000000 & 100.000000 & 1.2\% & 2.9\% & 1.1\% & 23.2\% & 6.3\% & 0.4\% & 1.1\% & 0.9\% & 0.7\% & 0.5\% & 0.5\% & 0.4\% & 0.4\% & 0.3\% \\
Cloud & 1024.000000 & 200.000000 & 1.3\% & 2.1\% & 1.2\% & 26.9\% & 3.6\% & 0.4\% & 1.4\% & 1.0\% & 0.8\% & 0.6\% & 0.6\% & 0.4\% & 0.4\% & 0.4\% \\
Spam & 4601.000000 & 10.000000 & 6.0\% & 28.4\% & 1.8\% & 0.0\% & 50.7\% & 21.7\% & 1.6\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
Spam & 4601.000000 & 25.000000 & 3.5\% & 9.4\% & 2.0\% & 12.4\% & 296.9\% & 118.5\% & 2.1\% & 0.6\% & 0.5\% & 0.4\% & 0.4\% & 0.4\% & 0.4\% & 0.4\% \\
Spam & 4601.000000 & 50.000000 & 2.5\% & 6.2\% & 1.7\% & 245.4\% & 754.1\% & 133.7\% & 1.6\% & 1.0\% & 0.7\% & 0.6\% & 0.5\% & 0.5\% & 0.5\% & 0.5\% \\
Spam & 4601.000000 & 100.000000 & 2.2\% & 4.8\% & 1.5\% & 1635.4\% & 2042.9\% & 834.8\% & 1.1\% & 0.9\% & 0.7\% & 0.5\% & 0.5\% & 0.4\% & 0.4\% & 0.4\% \\
Spam & 4601.000000 & 200.000000 & 1.3\% & 4.6\% & 1.1\% & 5432.0\% & 4803.9\% & 2612.0\% & 1.2\% & 0.9\% & 0.5\% & 0.5\% & 0.4\% & 0.4\% & 0.4\% & 0.3\% \\
\midrule
Mean & nan & nan & 2.1\% & 5.4\% & 1.3\% & 9395.0\% & 532.2\% & 248.2\% & 1.3\% & 0.6\% & 0.5\% & 0.4\% & 0.4\% & 0.3\% & 0.3\% & 0.3\% \\
\toprule
\end{tabular}


==> coltables/msestd-opt.tex <==
\begin{tabular}{lrrrrrrrrrrrrrrrr}
\toprule
data set & n & k & kmpp1 & kmpp-orig1 & betterkmpp & \thead{Hartigan- \\ Wong} & ga & rs & bkm01 & bkm03 & bkm05 & bkm10 & bkm15 & bkm20 & bkm25 & bkm30 \\
\midrule
squares-3x3 & 225.000000 & 9.000000 & 15.8\% & 28.8\% & 0.0\% & 30.9\% & 0.2\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
squares-5x5 & 625.000000 & 25.000000 & 10.4\% & 15.3\% & 3.5\% & 18.7\% & 0.2\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
squares-7x7 & 1225.000000 & 49.000000 & 6.7\% & 9.6\% & 4.3\% & 12.3\% & 0.2\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
angles-3x3 & 1728.000000 & 27.000000 & 4.9\% & 9.8\% & 3.6\% & 15.2\% & 0.3\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
angles-5x5 & 2700.000000 & 75.000000 & 3.1\% & 6.7\% & 2.3\% & 10.1\% & 0.2\% & 0.1\% & 0.3\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
angles-7x7 & 3675.000000 & 147.000000 & 2.2\% & 4.7\% & 2.1\% & 7.8\% & 0.2\% & 0.4\% & 0.1\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
4squares-3x3 & 2304.000000 & 36.000000 & 4.0\% & 6.6\% & 3.0\% & 13.4\% & 0.3\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
4squares-5x5 & 3600.000000 & 100.000000 & 2.3\% & 4.5\% & 2.2\% & 8.2\% & 0.2\% & 0.1\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
4squares-7x7 & 4900.000000 & 196.000000 & 1.5\% & 3.2\% & 1.6\% & 5.7\% & 0.2\% & 0.4\% & 2.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
\midrule
Mean & nan & nan & 5.7\% & 9.9\% & 2.5\% & 13.6\% & 0.2\% & 0.1\% & 0.3\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
\toprule
\end{tabular}


==> coltables/t-msestd-espiralX.tex <==
\begin{table}[ht]
    \small
    \begin{center}
    \input{coltables/msestd-espiralX.tex}
    \caption{"Evil Spiral" problems: Standard deviations corresponding to the SSE improvements from Table \ref{tab:mse-top}. \tabcom}
    \label{tab:msestd-espiralX}
    \end{center}
\end{table}
\renewcommand{\tabcom}{}

==> coltables/t-msestd-fr-mod.tex <==
\begin{table}[ht]
    \small
    \begin{center}
    \input{coltables/msestd-fr-mod.tex}
    \caption{Modified literature problems: Standard deviations corresponding to the SSE improvements from Table \ref{tab:mse-top}. \tabcom}
    \label{tab:msestd-fr-mod}
    \end{center}
\end{table}
\renewcommand{\tabcom}{}

==> coltables/t-msestd-fraenti.tex <==
\begin{table}[ht]
    \small
    \begin{center}
    \input{coltables/msestd-fraenti.tex}
    \caption{Literature problems: Standard deviations corresponding to the SSE improvements from Table \ref{tab:mse-top}. \tabcom}
    \label{tab:msestd-fränti}
    \end{center}
\end{table}
\renewcommand{\tabcom}{}

==> coltables/t-msestd-high-D.tex <==
\begin{table}[ht]
    \small
    \begin{center}
    \input{coltables/msestd-high-D.tex}
    \caption{High-dimensional problems: Standard deviations corresponding to the SSE improvements from Table \ref{tab:mse-top}. \tabcom}
    \label{tab:msestd-high-D}
    \end{center}
\end{table}
\renewcommand{\tabcom}{}

==> coltables/t-msestd-opt.tex <==
\begin{table}[ht]
    \small
    \begin{center}
    \input{coltables/msestd-opt.tex}
    \caption{Problems with known optimum: Standard deviations corresponding to the SSE improvements from Table \ref{tab:mse-top}. \tabcom}
    \label{tab:msestd-opt}
    \end{center}
\end{table}
\renewcommand{\tabcom}{}

==> img/prob-highD.tex <==
\begin{figure}
	\centering
	\includegraphics[width=\fiwid\linewidth]{img/prob-highD.png}
	\caption[short caption]{\capProbHighD}
	\label{fig:prob-highD}
\end{figure}

==> img/prob-opt-detail.tex <==
\begin{figure}
	\centering
	\includegraphics[width=\fiwid\linewidth]{img/prob-opt-detail.png}
	\caption[short caption]{\capProbOptDetail}
	\label{fig:prob-opt-detail}
\end{figure}

==> tables/imgcode_u.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.999\linewidth]{imgG/Jain.png}
    \caption[short caption]{Data set "Jain", k=30}
\end{figure}
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.999\linewidth]{imgG/R15.png}
    \caption[short caption]{Data set "R15", k=30}
\end{figure}
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.999\linewidth]{imgG/D31.png}
    \caption[short caption]{Data set "D31", k=100}
\end{figure}
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.999\linewidth]{imgG/Aggregation.png}
    \caption[short caption]{Data set "Aggregation", k=200}
\end{figure}
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.999\linewidth]{imgG/Flame.png}
    \caption[short caption]{Data set "Flame", k=80}
\end{figure}
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.999\linewidth]{imgG/Spiral.png}
    \caption[short caption]{Data set "Spiral", k=80}
\end{figure}
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.999\linewidth]{imgG/S2.png}
    \caption[short caption]{Data set "S2", k=100}
\end{figure}
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.999\linewidth]{imgG/Unbalance.png}
    \caption[short caption]{Data set "Unbalance", k=100}
\end{figure}
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.999\linewidth]{imgG/Birch1.png}
    \caption[short caption]{Data set "Birch1", k=100}
\end{figure}
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.999\linewidth]{imgG/Birch3.png}
    \caption[short caption]{Data set "Birch3", k=100}
\end{figure}
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.999\linewidth]{imgG/gmd5x5.png}
    \caption[short caption]{Data set "gmd5x5", k=50}
\end{figure}
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.999\linewidth]{imgG/gmd8x8.png}
    \caption[short caption]{Data set "gmd8x8", k=128}
\end{figure}
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.999\linewidth]{imgG/noise.png}
    \caption[short caption]{Data set "noise", k=100}
\end{figure}
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.999\linewidth]{imgG/vardensity.png}
    \caption[short caption]{Data set "vardensity", k=100}
\end{figure}
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.999\linewidth]{imgG/uniform.png}
    \caption[short caption]{Data set "uniform", k=100}
\end{figure}
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.999\linewidth]{imgG/sq6x6-2x2.png}
    \caption[short caption]{Data set "sq6x6-2x2", k=144}
\end{figure}
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.999\linewidth]{imgG/randangles.png}
    \caption[short caption]{Data set "randangles", k=60}
\end{figure}
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.999\linewidth]{imgG/stains.png}
    \caption[short caption]{Data set "stains", k=100}
\end{figure}
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.999\linewidth]{imgG/correlated.png}
    \caption[short caption]{Data set "correlated", k=100}
\end{figure}
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.999\linewidth]{imgG/rice.png}
    \caption[short caption]{Data set "rice", k=120}
\end{figure}


==> tables/tabcpuCloud.tex <==

    %nogogo
    \begin{tabular}{lrrrr@{\hspace{0.2em}}r @{\hspace{0.2em}}rr@{\hspace{0.2em}}r@{\hspace{0.2em}}rrr}
	\toprule
	data set &       n &    d &    k &   \multicolumn{3}{c}{$\cpukmp$}  &   \multicolumn{3}{c}{$\cpubkm$} & $\delcpu$ \\
	\midrule
    
   Cloud &  1024 &  10 &   25 &  0.29s &  $\pm$ & 20.33\% &  0.16s &  $\pm$ & 22.93\% &  \textbf{45.8\%} \\
   Cloud &  1024 &  10 &   50 &  0.44s &  $\pm$ & 24.80\% &  0.19s &  $\pm$ & 23.02\% &  \textbf{56.9\%} \\
   Cloud &  1024 &  10 &  100 &  0.60s &  $\pm$ & 26.80\% &  0.27s &  $\pm$ & 20.49\% &  \textbf{54.6\%} \\
   Cloud &  1024 &  10 &  150 &  0.88s &  $\pm$ & 22.67\% &  0.41s &  $\pm$ & 28.11\% &  \textbf{53.1\%} \\
   Cloud &  1024 &  10 &  200 &  1.11s &  $\pm$ & 17.87\% &  0.58s &  $\pm$ & 25.63\% &  \textbf{48.0\%} \\
\midrule
 Average & & &       &     &      &        &            &        &            &  \textbf{51.6\%} \\
\bottomrule
\end{tabular}

==> tables/tabcpuIntrusion.tex <==

    %nogogo
    \begin{tabular}{lrrrr@{\hspace{0.2em}}r @{\hspace{0.2em}}rr@{\hspace{0.2em}}r@{\hspace{0.2em}}rrr}
	\toprule
	data set &       n &    d &    k &   \multicolumn{3}{c}{$\cpukmp$}  &   \multicolumn{3}{c}{$\cpubkm$} & $\delcpu$ \\
	\midrule
    
 Intrusion &  494021 &  35 &   25 &   16.66s &  $\pm$ & 4.58\% &  24.35s &  $\pm$ & 39.91\% &               -46.2\% \\
 Intrusion &  494021 &  35 &   50 &   31.02s &  $\pm$ & 3.56\% &  30.50s &  $\pm$ & 26.06\% &  \textbf{ 1.7\%} \\
 Intrusion &  494021 &  35 &  100 &   64.29s &  $\pm$ & 3.42\% &  56.20s &  $\pm$ & 21.06\% &  \textbf{12.6\%} \\
 Intrusion &  494021 &  35 &  150 &  100.80s &  $\pm$ & 3.35\% &  66.73s &  $\pm$ & 15.70\% &  \textbf{33.8\%} \\
 Intrusion &  494021 &  35 &  200 &  132.83s &  $\pm$ & 3.44\% &  80.59s &  $\pm$ & 19.14\% &  \textbf{39.3\%} \\
\midrule
   Average & & &         &     &      &          &           &         &            &  \textbf{ 8.2\%} \\
\bottomrule
\end{tabular}

==> tables/tabcpuLineseg.tex <==

    %nogogo
    \begin{tabular}{lrrrr@{\hspace{0.2em}}r @{\hspace{0.2em}}rr@{\hspace{0.2em}}r@{\hspace{0.2em}}rrr}
	\toprule
	data set &       n &    d &    k &   \multicolumn{3}{c}{\thead{$\cpukmpmean$}}  &   \multicolumn{3}{c}{\thead{$\cpubkmmean$}}  & \thead{$\delcpumean$} \\
	\midrule
    
 lineseg02 &  300 &  1 &   6 &  0.05s &  $\pm$ & 10.47\% &  0.10s &  $\pm$ &  7.89\% &      -84.6\% \\
 lineseg04 &  600 &  1 &  12 &  0.08s &   $\pm$ & 7.79\% &  0.16s &  $\pm$ &  6.72\% &      -95.8\% \\
\bottomrule
\end{tabular}


==> tables/tabcpuNorm25.tex <==

    %nogogo
    \begin{tabular}{lrrrr@{\hspace{0.2em}}r @{\hspace{0.2em}}rr@{\hspace{0.2em}}r@{\hspace{0.2em}}rrr}
	\toprule
	data set &       n &    d &    k &   \multicolumn{3}{c}{$\cpukmp$}  &   \multicolumn{3}{c}{$\cpubkm$} & $\delcpu$ \\
	\midrule
    
 Norm25-new &  10000 &  15 &   25 &  0.39s &  $\pm$ & 27.00\% &  0.17s &  $\pm$ & 18.88\% &  \textbf{55.9\%} \\
 Norm25-new &  10000 &  15 &   50 &  0.81s &  $\pm$ & 21.24\% &  0.54s &  $\pm$ & 13.99\% &  \textbf{33.4\%} \\
 Norm25-new &  10000 &  15 &  100 &  2.06s &  $\pm$ & 10.04\% &  0.95s &  $\pm$ & 15.42\% &  \textbf{53.6\%} \\
 Norm25-new &  10000 &  15 &  150 &  3.17s &   $\pm$ & 8.97\% &  2.14s &  $\pm$ & 20.13\% &  \textbf{32.4\%} \\
 Norm25-new &  10000 &  15 &  200 &  4.13s &   $\pm$ & 6.53\% &  2.80s &  $\pm$ & 14.96\% &  \textbf{32.3\%} \\
\midrule
    Average & & &        &     &      &        &            &        &            &  \textbf{41.5\%} \\
\bottomrule
\end{tabular}

==> tables/tabcpuSpam.tex <==

    %nogogo
    \begin{tabular}{lrrrr@{\hspace{0.2em}}r @{\hspace{0.2em}}rr@{\hspace{0.2em}}r@{\hspace{0.2em}}rrr}
	\toprule
	data set &       n &    d &    k &   \multicolumn{3}{c}{$\cpukmp$}  &   \multicolumn{3}{c}{$\cpubkm$} & $\delcpu$ \\
	\midrule
    
    Spam &  4601 &  58 &   25 &  0.52s &  $\pm$ & 25.82\% &  0.37s &  $\pm$ & 15.77\% &  \textbf{29.1\%} \\
    Spam &  4601 &  58 &   50 &  0.90s &  $\pm$ & 25.30\% &  0.53s &  $\pm$ & 17.98\% &  \textbf{40.8\%} \\
    Spam &  4601 &  58 &  100 &  1.60s &  $\pm$ & 19.25\% &  0.97s &  $\pm$ & 17.28\% &  \textbf{39.4\%} \\
    Spam &  4601 &  58 &  150 &  2.64s &  $\pm$ & 17.12\% &  1.74s &  $\pm$ & 24.82\% &  \textbf{34.1\%} \\
    Spam &  4601 &  58 &  200 &  3.45s &  $\pm$ & 10.34\% &  2.25s &  $\pm$ & 19.79\% &  \textbf{34.8\%} \\
\midrule
 Average & & &       &     &      &        &            &        &            &  \textbf{35.6\%} \\
\bottomrule
\end{tabular}

==> tables/tabcpuUnknown.tex <==

    %nogogo
    \begin{tabular}{lrrrr@{\hspace{0.2em}}r @{\hspace{0.2em}}rr@{\hspace{0.2em}}r@{\hspace{0.2em}}rrr}
	\toprule
	data set &       n &    d &    k &   \multicolumn{3}{c}{$\cpukmp$}  &   \multicolumn{3}{c}{$\cpubkm$} & $\delcpu$ \\
	\midrule
    
        Jain &     373 &  2 &   30 &   0.11s &   $\pm$ & 4.52\% &  0.06s &  $\pm$ & 15.47\% &  \textbf{47.6\%} \\
         R15 &     600 &  2 &   30 &   0.11s &   $\pm$ & 3.89\% &  0.07s &  $\pm$ & 16.41\% &  \textbf{41.5\%} \\
         D31 &    3100 &  2 &  100 &   0.64s &   $\pm$ & 4.82\% &  0.36s &  $\pm$ & 19.27\% &  \textbf{43.3\%} \\
 Aggregation &     788 &  2 &  200 &   0.83s &  $\pm$ & 15.07\% &  0.40s &  $\pm$ & 22.37\% &  \textbf{52.1\%} \\
       Flame &     240 &  2 &   80 &   0.22s &   $\pm$ & 2.75\% &  0.09s &  $\pm$ & 14.97\% &  \textbf{60.4\%} \\
      Spiral &     312 &  2 &   80 &   0.23s &   $\pm$ & 2.63\% &  0.08s &  $\pm$ & 12.88\% &  \textbf{67.1\%} \\
          S2 &    5000 &  2 &  100 &   1.15s &  $\pm$ & 16.72\% &  0.51s &  $\pm$ & 16.41\% &  \textbf{55.7\%} \\
   Unbalance &    6500 &  2 &  100 &   1.04s &  $\pm$ & 17.01\% &  0.49s &  $\pm$ & 18.77\% &  \textbf{53.2\%} \\
      Birch1 &  100000 &  2 &  100 &   9.21s &   $\pm$ & 5.69\% &  4.63s &  $\pm$ &  6.78\% &  \textbf{49.8\%} \\
      Birch3 &  100000 &  2 &  100 &  12.17s &   $\pm$ & 5.50\% &  8.03s &  $\pm$ & 16.86\% &  \textbf{34.0\%} \\
      gmd5x5 &   10000 &  2 &   50 &   0.63s &  $\pm$ & 20.90\% &  0.37s &  $\pm$ & 14.66\% &  \textbf{40.6\%} \\
      gmd8x8 &   25600 &  2 &  128 &   4.37s &   $\pm$ & 6.51\% &  2.49s &  $\pm$ & 17.76\% &  \textbf{43.0\%} \\
       noise &   13664 &  2 &  100 &   1.87s &  $\pm$ & 10.00\% &  0.89s &  $\pm$ & 15.21\% &  \textbf{52.2\%} \\
  vardensity &   30000 &  2 &  100 &   4.86s &   $\pm$ & 5.40\% &  2.60s &  $\pm$ & 17.49\% &  \textbf{46.5\%} \\
     uniform &    1000 &  2 &  100 &   0.40s &   $\pm$ & 5.67\% &  0.20s &  $\pm$ & 21.09\% &  \textbf{51.0\%} \\
   sq6x6-2x2 &    3600 &  2 &  144 &   1.06s &  $\pm$ & 12.51\% &  0.39s &  $\pm$ & 21.37\% &  \textbf{63.4\%} \\
  randangles &    3840 &  2 &   60 &   0.38s &   $\pm$ & 5.69\% &  0.16s &  $\pm$ & 14.23\% &  \textbf{57.4\%} \\
      stains &   10000 &  2 &  100 &   1.42s &  $\pm$ & 11.98\% &  0.68s &  $\pm$ & 18.25\% &  \textbf{52.3\%} \\
  correlated &    6000 &  2 &  100 &   1.24s &  $\pm$ & 16.08\% &  0.56s &  $\pm$ & 16.74\% &  \textbf{54.9\%} \\
        rice &   10000 &  2 &  120 &   1.36s &  $\pm$ & 13.82\% &  0.57s &  $\pm$ & 12.66\% &  \textbf{58.4\%} \\
\midrule
     Average & & &         &    &      &         &            &        &            &  \textbf{51.2\%} \\
\bottomrule
\end{tabular}

==> tables/tabmulCloud.tex <==
\begin{tabular}{llrrrrrrrr}
\toprule
data set &    k & $\phi_{kmp}^{min}$ & $\phi_{bkm}^{min}$ &  $\Tkmp$ &  $\Tbkm$ &  $\#_{kmp}$ &  $\#_{bkm}$ &            $imp^{tot}$ &             $\overline{imp}$ \\
\midrule
 Cloud &   10 &   5.762E+06 &   5.762E+06 &  11.8s &  11.7s &     100 &      76 &               -0.00\% &               -0.13\% \\
 Cloud &   25 &   1.958E+06 &   1.955E+06 &  18.3s &  18.2s &      90 &     100 &  \textbf{0.14\%} &  \textbf{1.43\%} \\
 Cloud &   50 &   1.071E+06 &   1.054E+06 &  23.5s &  23.3s &      69 &     100 &  \textbf{1.60\%} &  \textbf{2.34\%} \\
 Cloud &  100 &   5.992E+05 &   5.795E+05 &  35.4s &  35.0s &      57 &     100 &  \textbf{3.28\%} &  \textbf{3.08\%} \\
 Cloud &  150 &   4.043E+05 &   3.899E+05 &  49.8s &  49.6s &      54 &     100 &  \textbf{3.56\%} &  \textbf{3.44\%} \\
 Cloud &  200 &   2.933E+05 &   2.841E+05 &  65.7s &  64.9s &      55 &     100 &  \textbf{3.16\%} &  \textbf{3.65\%} \\
\bottomrule
\end{tabular}


==> tables/tabmulIntrusion.tex <==
\begin{tabular}{llrrrrrrrr}
\toprule
    data set &    k & $\phi_{kmp}^{min}$ & $\phi_{bkm}^{min}$ &    $\Tkmp$ &    $\Tbkm$ &  $\#_{kmp}$ &  $\#_{bkm}$ &            $imp^{tot}$ &             $\overline{imp}$ \\
\midrule
 Intrusion &   10 &   1.158E+13 &   1.158E+13 &   943.1s &   925.9s &     100 &      37 &                0.00\% &  \textbf{0.06\%} \\
 Intrusion &   25 &   1.070E+12 &   1.071E+12 &  2400.8s &  2386.4s &     100 &      54 &               -0.09\% &  \textbf{1.06\%} \\
 Intrusion &   50 &   1.968E+11 &   1.941E+11 &  4352.4s &  4309.2s &     100 &      83 &  \textbf{1.39\%} &  \textbf{3.08\%} \\
 Intrusion &  100 &   3.790E+10 &   3.676E+10 &  6654.8s &  6600.8s &      69 &     100 &  \textbf{3.02\%} &  \textbf{3.20\%} \\
 Intrusion &  150 &   1.417E+10 &   1.358E+10 &  8111.8s &  8071.9s &      50 &     100 &  \textbf{4.20\%} &  \textbf{2.20\%} \\
 Intrusion &  200 &   7.453E+09 &   7.141E+09 &  9837.9s &  9634.3s &      47 &     100 &  \textbf{4.18\%} &  \textbf{2.03\%} \\
\bottomrule
\end{tabular}


==> tables/tabmulNorm25.tex <==
\begin{tabular}{llrrrrrrrr}
\toprule
     data set &    k & $\phi_{kmp}^{min}$ & $\phi_{bkm}^{min}$ &   $\Tkmp$ &   $\Tbkm$ &  $\#_{kmp}$ &  $\#_{bkm}$ &            $imp^{tot}$ &             $\overline{imp}$ \\
\midrule
 Norm25-new &   10 &   1.041E+09 &   1.041E+09 &   30.8s &   30.3s &     100 &      30 &               -0.02\% &  \textbf{1.53\%} \\
 Norm25-new &   25 &   1.491E+05 &   1.491E+05 &   73.9s &   73.9s &     100 &      95 &                0.00\% &                0.00\% \\
 Norm25-new &   50 &   1.417E+05 &   1.405E+05 &  129.2s &  128.5s &     100 &      57 &  \textbf{0.91\%} &  \textbf{0.88\%} \\
 Norm25-new &  100 &   1.306E+05 &   1.297E+05 &  286.3s &  285.0s &     100 &      87 &  \textbf{0.74\%} &  \textbf{0.82\%} \\
 Norm25-new &  150 &   1.231E+05 &   1.225E+05 &  362.3s &  362.3s &     100 &      98 &  \textbf{0.52\%} &  \textbf{0.63\%} \\
 Norm25-new &  200 &   1.175E+05 &   1.168E+05 &  441.1s &  436.8s &      95 &     100 &  \textbf{0.61\%} &  \textbf{0.56\%} \\
\bottomrule
\end{tabular}


==> tables/tabmulSpam.tex <==
\begin{tabular}{llrrrrrrrr}
\toprule
data set &    k & $\phi_{kmp}^{min}$ & $\phi_{bkm}^{min}$ &   $\Tkmp$ &   $\Tbkm$ &  $\#_{kmp}$ &  $\#_{bkm}$ &            $imp^{tot}$ &             $\overline{imp}$ \\
\midrule
  Spam &   10 &   7.698E+07 &   7.698E+07 &   38.9s &   37.9s &     100 &      48 &               -0.00\% &  \textbf{0.02\%} \\
  Spam &   25 &   1.524E+07 &   1.524E+07 &   73.5s &   72.6s &     100 &      79 &  \textbf{0.05\%} &  \textbf{0.64\%} \\
  Spam &   50 &   5.711E+06 &   5.707E+06 &  117.9s &  117.5s &      96 &     100 &  \textbf{0.07\%} &  \textbf{2.37\%} \\
  Spam &  100 &   2.032E+06 &   1.987E+06 &  188.7s &  186.9s &      86 &     100 &  \textbf{2.18\%} &  \textbf{3.15\%} \\
  Spam &  150 &   1.031E+06 &   1.000E+06 &  255.8s &  253.3s &      80 &     100 &  \textbf{2.99\%} &  \textbf{3.21\%} \\
  Spam &  200 &   6.504E+05 &   6.371E+05 &  303.4s &  301.5s &      75 &     100 &  \textbf{2.05\%} &  \textbf{2.56\%} \\
\bottomrule
\end{tabular}


==> tables/tabmulUnknown.tex <==
\begin{tabular}{llrrrrrrrr}
\toprule
      data set &    k & $\phi_{kmp}^{min}$ & $\phi_{bkm}^{min}$ &    $\Tkmp$ &    $\Tbkm$ &  $\#_{kmp}$ &  $\#_{bkm}$ &            $imp^{tot}$ &             $\overline{imp}$ \\
\midrule
        Jain &   30 &   5.887E+02 &   5.770E+02 &    10.0s &    10.0s &      54 &     100 &  \textbf{1.99\%} &  \textbf{3.05\%} \\
         R15 &   30 &   6.591E+01 &   6.523E+01 &    12.0s &    12.1s &      62 &     100 &  \textbf{1.03\%} &  \textbf{3.09\%} \\
         D31 &  100 &   1.341E+03 &   1.313E+03 &    79.3s &    79.6s &      68 &     100 &  \textbf{2.08\%} &  \textbf{3.12\%} \\
 Aggregation &  200 &   2.457E+02 &   2.313E+02 &    46.4s &    46.4s &      39 &     100 &  \textbf{5.89\%} &  \textbf{5.04\%} \\
       Flame &   80 &   4.574E+01 &   4.339E+01 &    13.6s &    13.7s &      34 &     100 &  \textbf{5.15\%} &  \textbf{6.65\%} \\
      Spiral &   80 &   1.244E+02 &   1.194E+02 &    12.4s &    12.4s &      31 &     100 &  \textbf{3.98\%} &  \textbf{3.17\%} \\
          S2 &  100 &   2.629E+12 &   2.581E+12 &   106.9s &   108.1s &      76 &     100 &  \textbf{1.85\%} &  \textbf{2.09\%} \\
   Unbalance &  100 &   2.337E+10 &   2.278E+10 &    97.6s &    98.5s &      77 &     100 &  \textbf{2.56\%} &  \textbf{3.11\%} \\
      Birch1 &  100 &   9.509E+13 &   9.277E+13 &   840.7s &   846.4s &      67 &     100 &  \textbf{2.43\%} &  \textbf{4.39\%} \\
      Birch3 &  100 &   3.759E+13 &   3.717E+13 &  1391.0s &  1405.1s &      87 &     100 &  \textbf{1.13\%} &  \textbf{1.61\%} \\
      gmd5x5 &   50 &   6.328E+00 &   6.148E+00 &    83.1s &    82.7s &     100 &      90 &  \textbf{2.85\%} &  \textbf{6.81\%} \\
      gmd8x8 &  128 &   5.528E+00 &   5.228E+00 &   318.8s &   321.7s &      83 &     100 &  \textbf{5.41\%} &  \textbf{8.18\%} \\
       noise &  100 &   1.066E+01 &   1.058E+01 &   178.4s &   180.5s &      72 &     100 &  \textbf{0.76\%} &  \textbf{3.18\%} \\
  vardensity &  100 &   2.603E+01 &   2.579E+01 &   442.1s &   447.5s &      78 &     100 &  \textbf{0.92\%} &  \textbf{1.28\%} \\
     uniform &  100 &   1.234E+00 &   1.191E+00 &    26.3s &    26.5s &      44 &     100 &  \textbf{3.51\%} &  \textbf{3.63\%} \\
   sq6x6-2x2 &  144 &   2.101E+00 &   2.041E+00 &    65.2s &    66.0s &      45 &     100 &  \textbf{2.85\%} &  \textbf{7.14\%} \\
  randangles &   60 &   3.384E+00 &   3.272E+00 &    40.3s &    40.7s &      63 &     100 &  \textbf{3.30\%} &  \textbf{5.85\%} \\
      stains &  100 &   5.457E+05 &   5.374E+05 &   139.0s &   140.5s &      79 &     100 &  \textbf{1.51\%} &  \textbf{2.53\%} \\
  correlated &  100 &   5.531E+05 &   5.463E+05 &   104.1s &   105.2s &      68 &     100 &  \textbf{1.22\%} &  \textbf{2.01\%} \\
        rice &  120 &   2.597E+05 &   2.534E+05 &   128.0s &   128.7s &      76 &     100 &  \textbf{2.41\%} &  \textbf{4.53\%} \\
\bottomrule
\end{tabular}


==> tables/taboptLineseg.tex <==

\begin{tabular}{lrrrrr@{\hspace{0.2em}}r @{\hspace{0.2em}}rr@{\hspace{0.2em}}r@{\hspace{0.2em}}rr}
\toprule
data set &       n &    d & k & optimum & \multicolumn{3}{c}{\thead{$\deloptkmp$}}  &   \multicolumn{3}{c}{\thead{$\deloptbkm$}}&{\thead{$\delssemean$}}   \\
\midrule
    
 lineseg02 &  300 &  1 &   6 &   0.444267 &  0.07\% &  $\pm$ &0.03\% &  \textbf{0.06\%} &  $\pm$ &0.02\% &                0.01\% \\
 lineseg04 &  600 &  1 &  12 &   0.222133 &  0.65\% &  $\pm$ &2.04\% &  \textbf{0.08\%} &  $\pm$ &0.02\% &  \textbf{0.57\%} \\
\bottomrule
\end{tabular}


==> tables/tabretCloud.tex <==

    %nogogo
    \begin{tabular}{lrrrr r@{\hspace{0.2em}}r@{\hspace{0.2em}}rr}
	\toprule
	data set &       n &    d &  k &  $\ssekmpmean$  &   \multicolumn{3}{c}{\thead{$\ssebkmmean$}}  & \thead{$\delssemean$} \\
	\midrule
    
 Cloud &  1024 &  10 &   10 & 5.762E+06 & 5.783E+06 &  $\pm$ &0.44\% &               -0.36\% \\
 Cloud &  1024 &  10 &   25 & 1.958E+06 & 1.975E+06 &  $\pm$ &0.76\% &               -0.87\% \\
 Cloud &  1024 &  10 &   50 & 1.071E+06 & 1.064E+06 &  $\pm$ &0.65\% &  \textbf{0.66\%} \\
 Cloud &  1024 &  10 &  100 & 5.992E+05 & 5.900E+05 &  $\pm$ &0.87\% &  \textbf{1.53\%} \\
 Cloud &  1024 &  10 &  150 & 4.035E+05 & 3.968E+05 &  $\pm$ &0.84\% &  \textbf{1.68\%} \\
 Cloud &  1024 &  10 &  200 & 2.933E+05 & 2.896E+05 &  $\pm$ &0.86\% &  \textbf{1.28\%} \\
\bottomrule
\end{tabular}


==> tables/tabretIntrusion.tex <==

    %nogogo
    \begin{tabular}{lrrrr r@{\hspace{0.2em}}r@{\hspace{0.2em}}rr}
	\toprule
	data set &       n &    d &  k &  $\ssekmpmean$  &   \multicolumn{3}{c}{\thead{$\ssebkmmean$}}  & \thead{$\delssemean$} \\
	\midrule
    
 Intrusion &  494021 &  35 &   10 & 1.158E+13 & 1.158E+13 &  $\pm$ &0.20\% &               -0.03\% \\
 Intrusion &  494021 &  35 &   25 & 1.070E+12 & 1.089E+12 &  $\pm$ &1.84\% &               -1.73\% \\
 Intrusion &  494021 &  35 &   50 & 1.968E+11 & 1.986E+11 &  $\pm$ &1.55\% &               -0.94\% \\
 Intrusion &  494021 &  35 &  100 & 3.790E+10 & 3.756E+10 &  $\pm$ &1.36\% &  \textbf{0.89\%} \\
 Intrusion &  494021 &  35 &  150 & 1.417E+10 & 1.420E+10 &  $\pm$ &2.46\% &               -0.21\% \\
 Intrusion &  494021 &  35 &  200 & 7.413E+09 & 7.401E+09 &  $\pm$ &2.04\% &  \textbf{0.17\%} \\
\bottomrule
\end{tabular}


==> tables/tabretNorm25.tex <==

    %nogogo
    \begin{tabular}{lrrrr r@{\hspace{0.2em}}r@{\hspace{0.2em}}rr}
	\toprule
	data set &       n &    d &  k &  $\ssekmpmean$  &   \multicolumn{3}{c}{\thead{$\ssebkmmean$}}  & \thead{$\delssemean$} \\
	\midrule
    
 Norm25-new &  10000 &  15 &   10 & 1.041E+09 & 1.081E+09 &  $\pm$ &2.61\% &               -3.79\% \\
 Norm25-new &  10000 &  15 &   25 & 1.491E+05 & 1.491E+05 &  $\pm$ &0.00\% &               -0.00\% \\
 Norm25-new &  10000 &  15 &   50 & 1.417E+05 & 1.408E+05 &  $\pm$ &0.08\% &  \textbf{0.67\%} \\
 Norm25-new &  10000 &  15 &  100 & 1.306E+05 & 1.299E+05 &  $\pm$ &0.10\% &  \textbf{0.54\%} \\
 Norm25-new &  10000 &  15 &  150 & 1.231E+05 & 1.227E+05 &  $\pm$ &0.12\% &  \textbf{0.34\%} \\
 Norm25-new &  10000 &  15 &  200 & 1.175E+05 & 1.172E+05 &  $\pm$ &0.12\% &  \textbf{0.27\%} \\
\bottomrule
\end{tabular}


==> tables/tabretSpam.tex <==

    %nogogo
    \begin{tabular}{lrrrr r@{\hspace{0.2em}}r@{\hspace{0.2em}}rr}
	\toprule
	data set &       n &    d &  k &  $\ssekmpmean$  &   \multicolumn{3}{c}{\thead{$\ssebkmmean$}}  & \thead{$\delssemean$} \\
	\midrule
    
  Spam &  4601 &  58 &   10 & 7.698E+07 & 7.698E+07 &  $\pm$ &0.01\% &               -0.00\% \\
  Spam &  4601 &  58 &   25 & 1.524E+07 & 1.541E+07 &  $\pm$ &0.73\% &               -1.08\% \\
  Spam &  4601 &  58 &   50 & 5.711E+06 & 5.788E+06 &  $\pm$ &0.91\% &               -1.35\% \\
  Spam &  4601 &  58 &  100 & 2.032E+06 & 2.009E+06 &  $\pm$ &0.75\% &  \textbf{1.13\%} \\
  Spam &  4601 &  58 &  150 & 1.030E+06 & 1.017E+06 &  $\pm$ &0.71\% &  \textbf{1.26\%} \\
  Spam &  4601 &  58 &  200 & 6.504E+05 & 6.479E+05 &  $\pm$ &0.86\% &  \textbf{0.39\%} \\
\bottomrule
\end{tabular}


==> tables/tabretUnknown.tex <==

    %nogogo
    \begin{tabular}{lrrrr r@{\hspace{0.2em}}r@{\hspace{0.2em}}rr}
	\toprule
	data set &       n &    d &  k &  $\ssekmpmean$  &   \multicolumn{3}{c}{\thead{$\ssebkmmean$}}  & \thead{$\delssemean$} \\
	\midrule
    
        Jain &     373 &  2 &   30 & 5.864E+02 & 5.864E+02 &  $\pm$ &1.12\% &               -0.00\% \\
         R15 &     600 &  2 &   30 & 6.591E+01 & 6.589E+01 &  $\pm$ &0.51\% &  \textbf{0.03\%} \\
         D31 &    3100 &  2 &  100 & 1.341E+03 & 1.325E+03 &  $\pm$ &0.41\% &  \textbf{1.19\%} \\
 Aggregation &     788 &  2 &  200 & 2.457E+02 & 2.372E+02 &  $\pm$ &1.21\% &  \textbf{3.46\%} \\
       Flame &     240 &  2 &   80 & 4.574E+01 & 4.475E+01 &  $\pm$ &1.69\% &  \textbf{2.16\%} \\
      Spiral &     312 &  2 &   80 & 1.242E+02 & 1.230E+02 &  $\pm$ &1.33\% &  \textbf{0.92\%} \\
          S2 &    5000 &  2 &  100 & 2.629E+12 & 2.605E+12 &  $\pm$ &0.46\% &  \textbf{0.91\%} \\
   Unbalance &    6500 &  2 &  100 & 2.337E+10 & 2.309E+10 &  $\pm$ &0.79\% &  \textbf{1.21\%} \\
      Birch1 &  100000 &  2 &  100 & 9.509E+13 & 9.278E+13 &  $\pm$ &0.00\% &  \textbf{2.43\%} \\
      Birch3 &  100000 &  2 &  100 & 3.759E+13 & 3.741E+13 &  $\pm$ &0.31\% &  \textbf{0.49\%} \\
      gmd5x5 &   10000 &  2 &   50 & 6.328E+00 & 6.151E+00 &  $\pm$ &0.23\% &  \textbf{2.80\%} \\
      gmd8x8 &   25600 &  2 &  128 & 5.528E+00 & 5.231E+00 &  $\pm$ &0.02\% &  \textbf{5.36\%} \\
       noise &   13664 &  2 &  100 & 1.066E+01 & 1.061E+01 &  $\pm$ &0.17\% &  \textbf{0.44\%} \\
  vardensity &   30000 &  2 &  100 & 2.592E+01 & 2.591E+01 &  $\pm$ &0.25\% &  \textbf{0.04\%} \\
     uniform &    1000 &  2 &  100 & 1.231E+00 & 1.211E+00 &  $\pm$ &0.91\% &  \textbf{1.63\%} \\
   sq6x6-2x2 &    3600 &  2 &  144 & 2.101E+00 & 2.041E+00 &  $\pm$ &0.00\% &  \textbf{2.85\%} \\
  randangles &    3840 &  2 &   60 & 3.384E+00 & 3.272E+00 &  $\pm$ &0.00\% &  \textbf{3.30\%} \\
      stains &   10000 &  2 &  100 & 5.457E+05 & 5.404E+05 &  $\pm$ &0.27\% &  \textbf{0.97\%} \\
  correlated &    6000 &  2 &  100 & 5.531E+05 & 5.528E+05 &  $\pm$ &0.62\% &  \textbf{0.05\%} \\
        rice &   10000 &  2 &  120 & 2.584E+05 & 2.573E+05 &  $\pm$ &0.86\% &  \textbf{0.46\%} \\
\bottomrule
\end{tabular}


==> tables/tabsseAllesRand.tex <==

    %nogogo
    \begin{tabular}{lrrrr@{\hspace{0.2em}}r @{\hspace{0.2em}}rr@{\hspace{0.2em}}r@{\hspace{0.2em}}rr}
	\toprule
	data set &       n &    d &  k &  \multicolumn{3}{c}{\thead{$\ssekmpmean$}}  &   \multicolumn{3}{c}{\thead{$\ssebkmmean$}}  & \thead{$\delssemean$} \\
	\midrule
    
        Jain &     373 &  2 &   30 &       605.37 &  $\pm$ &1.34\% &       583.61 &  $\pm$ &0.85\% &  \textbf{3.59\%} \\
         R15 &     600 &  2 &   30 &        67.96 &  $\pm$ &1.12\% &        65.76 &  $\pm$ &0.36\% &  \textbf{3.23\%} \\
         D31 &    3100 &  2 &  100 &     1,367.01 &  $\pm$ &0.61\% &     1,323.89 &  $\pm$ &0.35\% &  \textbf{3.15\%} \\
 Aggregation &     788 &  2 &  200 &       249.68 &  $\pm$ &0.83\% &       233.50 &  $\pm$ &1.35\% &  \textbf{6.48\%} \\
       Flame &     240 &  2 &   80 &        48.02 &  $\pm$ &1.18\% &        44.02 &  $\pm$ &1.52\% &  \textbf{8.35\%} \\
      Spiral &     312 &  2 &   80 &       127.22 &  $\pm$ &1.21\% &       121.49 &  $\pm$ &1.28\% &  \textbf{4.50\%} \\
          S2 &    5000 &  2 &  100 &    2.662E+12 &  $\pm$ &0.43\% &    2.600E+12 &  $\pm$ &0.51\% &  \textbf{2.33\%} \\
   Unbalance &    6500 &  2 &  100 &    2.382E+10 &  $\pm$ &0.81\% &    2.286E+10 &  $\pm$ &0.61\% &  \textbf{4.02\%} \\
      Birch1 &  100000 &  2 &  100 &    9.696E+13 &  $\pm$ &1.62\% &    9.278E+13 &  $\pm$ &0.00\% &  \textbf{4.31\%} \\
      Birch3 &  100000 &  2 &  100 &    3.794E+13 &  $\pm$ &0.53\% &    3.743E+13 &  $\pm$ &0.28\% &  \textbf{1.36\%} \\
      gmd5x5 &   10000 &  2 &   50 &       6.6066 &  $\pm$ &1.64\% &       6.1494 &  $\pm$ &0.01\% &  \textbf{6.92\%} \\
      gmd8x8 &   25600 &  2 &  128 &       5.6984 &  $\pm$ &1.16\% &       5.2306 &  $\pm$ &0.02\% &  \textbf{8.21\%} \\
       noise &   13664 &  2 &   85 &        14.12 &  $\pm$ &0.92\% &        13.69 &  $\pm$ &0.20\% &  \textbf{3.09\%} \\
  vardensity &   30000 &  2 &  100 &        26.24 &  $\pm$ &0.35\% &        25.90 &  $\pm$ &0.23\% &  \textbf{1.28\%} \\
     uniform &    1000 &  2 &  100 &       1.2623 &  $\pm$ &0.79\% &       1.2034 &  $\pm$ &0.94\% &  \textbf{4.67\%} \\
   sq6x6-2x2 &    3600 &  2 &  144 &       2.1987 &  $\pm$ &1.08\% &       2.0409 &  $\pm$ &0.01\% &  \textbf{7.18\%} \\
  randangles &    3840 &  2 &   60 &       3.4589 &  $\pm$ &1.86\% &       3.2725 &  $\pm$ &0.00\% &  \textbf{5.39\%} \\
      stains &   10000 &  2 &   30 & 3,242,614.61 &  $\pm$ &1.83\% & 3,165,112.99 &  $\pm$ &0.01\% &  \textbf{2.39\%} \\
  correlated &    6000 &  2 &  100 &   563,522.04 &  $\pm$ &0.62\% &   551,586.25 &  $\pm$ &0.54\% &  \textbf{2.12\%} \\
        rice &   10000 &  2 &   80 &   746,018.97 &  $\pm$ &1.44\% &   713,703.98 &  $\pm$ &1.13\% &  \textbf{4.33\%} \\
\bottomrule
\end{tabular}


==> tables/tabsseCloud.tex <==

    %nogogo
    \begin{tabular}{lrrrr@{\hspace{0.2em}}r @{\hspace{0.2em}}rr@{\hspace{0.2em}}r@{\hspace{0.2em}}rr}
	\toprule
	data set &       n &    d &  k &  \multicolumn{3}{c}{$\ssekmp$}  &   \multicolumn{3}{c}{$\ssebkm$}  & $\delsse$\\
	\midrule
    
   Cloud &  1024 &  10 &   25 & 2.001E+06 &  $\pm$ &1.02\% & 1.973E+06 &  $\pm$ &0.73\% &  \textbf{1.41\%} \\
   Cloud &  1024 &  10 &   50 & 1.090E+06 &  $\pm$ &0.83\% & 1.062E+06 &  $\pm$ &0.55\% &  \textbf{2.51\%} \\
   Cloud &  1024 &  10 &  100 & 6.082E+05 &  $\pm$ &0.74\% & 5.865E+05 &  $\pm$ &0.81\% &  \textbf{3.57\%} \\
   Cloud &  1024 &  10 &  150 & 4.109E+05 &  $\pm$ &0.63\% & 3.946E+05 &  $\pm$ &0.79\% &  \textbf{3.97\%} \\
   Cloud &  1024 &  10 &  200 & 3.005E+05 &  $\pm$ &0.58\% & 2.866E+05 &  $\pm$ &0.72\% &  \textbf{4.63\%} \\
\midrule
 Average &     0 &   0 &    0 & 0.000E+00 &  $\pm$ &0.00\% & 0.000E+00 &  $\pm$ &0.00\% &  \textbf{3.22\%} \\
\bottomrule
\end{tabular}

==> tables/tabsseIntrusion.tex <==

    %nogogo
    \begin{tabular}{lrrrr@{\hspace{0.2em}}r @{\hspace{0.2em}}rr@{\hspace{0.2em}}r@{\hspace{0.2em}}rr}
	\toprule
	data set &       n &    d &  k &  \multicolumn{3}{c}{$\ssekmp$}  &   \multicolumn{3}{c}{$\ssebkm$}  & $\delsse$\\
	\midrule
    
 Intrusion &  494021 &  35 &   25 & 1.098E+12 &  $\pm$ &1.89\% & 1.088E+12 &  $\pm$ &1.89\% &  \textbf{0.94\%} \\
 Intrusion &  494021 &  35 &   50 & 2.052E+11 &  $\pm$ &1.70\% & 1.991E+11 &  $\pm$ &2.03\% &  \textbf{3.00\%} \\
 Intrusion &  494021 &  35 &  100 & 3.890E+10 &  $\pm$ &1.16\% & 3.720E+10 &  $\pm$ &0.98\% &  \textbf{4.39\%} \\
 Intrusion &  494021 &  35 &  150 & 1.453E+10 &  $\pm$ &1.18\% & 1.396E+10 &  $\pm$ &1.22\% &  \textbf{3.92\%} \\
 Intrusion &  494021 &  35 &  200 & 7.561E+09 &  $\pm$ &0.89\% & 7.330E+09 &  $\pm$ &1.82\% &  \textbf{3.06\%} \\
\midrule
   Average &       0 &   0 &    0 & 0.000E+00 &  $\pm$ &0.00\% & 0.000E+00 &  $\pm$ &0.00\% &  \textbf{3.06\%} \\
\bottomrule
\end{tabular}

==> tables/tabsseNorm25.tex <==

    %nogogo
    \begin{tabular}{lrrrr@{\hspace{0.2em}}r @{\hspace{0.2em}}rr@{\hspace{0.2em}}r@{\hspace{0.2em}}rr}
	\toprule
	data set &       n &    d &  k &  \multicolumn{3}{c}{$\ssekmp$}  &   \multicolumn{3}{c}{$\ssebkm$}  & $\delsse$\\
	\midrule
    
 Norm25-new &  10000 &  15 &   25 & 1.491E+05 &  $\pm$ &0.00\% & 1.491E+05 &  $\pm$ &0.00\% &                0.00\% \\
 Norm25-new &  10000 &  15 &   50 & 1.421E+05 &  $\pm$ &0.09\% & 1.405E+05 &  $\pm$ &0.06\% &  \textbf{1.09\%} \\
 Norm25-new &  10000 &  15 &  100 & 1.310E+05 &  $\pm$ &0.08\% & 1.299E+05 &  $\pm$ &0.08\% &  \textbf{0.90\%} \\
 Norm25-new &  10000 &  15 &  150 & 1.235E+05 &  $\pm$ &0.08\% & 1.225E+05 &  $\pm$ &0.12\% &  \textbf{0.78\%} \\
 Norm25-new &  10000 &  15 &  200 & 1.178E+05 &  $\pm$ &0.08\% & 1.170E+05 &  $\pm$ &0.13\% &  \textbf{0.74\%} \\
\midrule
    Average &      0 &   0 &    0 & 0.000E+00 &  $\pm$ &0.00\% & 0.000E+00 &  $\pm$ &0.00\% &  \textbf{0.70\%} \\
\bottomrule
\end{tabular}

==> tables/tabsseSpam.tex <==

    %nogogo
    \begin{tabular}{lrrrr@{\hspace{0.2em}}r @{\hspace{0.2em}}rr@{\hspace{0.2em}}r@{\hspace{0.2em}}rr}
	\toprule
	data set &       n &    d &  k &  \multicolumn{3}{c}{$\ssekmp$}  &   \multicolumn{3}{c}{$\ssebkm$}  & $\delsse$\\
	\midrule
    
    Spam &  4601 &  58 &   25 & 1.553E+07 &  $\pm$ &1.24\% & 1.540E+07 &  $\pm$ &0.47\% &  \textbf{0.83\%} \\
    Spam &  4601 &  58 &   50 & 5.917E+06 &  $\pm$ &1.36\% & 5.770E+06 &  $\pm$ &0.78\% &  \textbf{2.49\%} \\
    Spam &  4601 &  58 &  100 & 2.075E+06 &  $\pm$ &0.94\% & 2.011E+06 &  $\pm$ &0.76\% &  \textbf{3.08\%} \\
    Spam &  4601 &  58 &  150 & 1.050E+06 &  $\pm$ &0.81\% & 1.014E+06 &  $\pm$ &0.70\% &  \textbf{3.41\%} \\
    Spam &  4601 &  58 &  200 & 6.649E+05 &  $\pm$ &0.69\% & 6.470E+05 &  $\pm$ &0.73\% &  \textbf{2.69\%} \\
\midrule
 Average &     0 &   0 &    0 & 0.000E+00 &  $\pm$ &0.00\% & 0.000E+00 &  $\pm$ &0.00\% &  \textbf{2.50\%} \\
\bottomrule
\end{tabular}

==> tables/tabsseUnknown.tex <==

    %nogogo
    \begin{tabular}{lrrrr@{\hspace{0.2em}}r @{\hspace{0.2em}}rr@{\hspace{0.2em}}r@{\hspace{0.2em}}rr}
	\toprule
	data set &       n &    d &  k &  \multicolumn{3}{c}{$\ssekmp$}  &   \multicolumn{3}{c}{$\ssebkm$}  & $\delsse$\\
	\midrule
    
        Jain &     373 &  2 &   30 & 6.041E+02 &  $\pm$ &1.42\% & 5.835E+02 &  $\pm$ &0.88\% &  \textbf{3.40\%} \\
         R15 &     600 &  2 &   30 & 6.798E+01 &  $\pm$ &1.08\% & 6.580E+01 &  $\pm$ &0.44\% &  \textbf{3.21\%} \\
         D31 &    3100 &  2 &  100 & 1.367E+03 &  $\pm$ &0.58\% & 1.324E+03 &  $\pm$ &0.34\% &  \textbf{3.19\%} \\
 Aggregation &     788 &  2 &  200 & 2.499E+02 &  $\pm$ &0.76\% & 2.340E+02 &  $\pm$ &1.17\% &  \textbf{6.34\%} \\
       Flame &     240 &  2 &   80 & 4.792E+01 &  $\pm$ &1.34\% & 4.392E+01 &  $\pm$ &1.52\% &  \textbf{8.33\%} \\
      Spiral &     312 &  2 &   80 & 1.276E+02 &  $\pm$ &1.19\% & 1.220E+02 &  $\pm$ &1.19\% &  \textbf{4.40\%} \\
          S2 &    5000 &  2 &  100 & 2.665E+12 &  $\pm$ &0.50\% & 2.604E+12 &  $\pm$ &0.46\% &  \textbf{2.29\%} \\
   Unbalance &    6500 &  2 &  100 & 2.379E+10 &  $\pm$ &0.72\% & 2.300E+10 &  $\pm$ &0.75\% &  \textbf{3.33\%} \\
      Birch1 &  100000 &  2 &  100 & 9.664E+13 &  $\pm$ &1.31\% & 9.278E+13 &  $\pm$ &0.00\% &  \textbf{3.99\%} \\
      Birch3 &  100000 &  2 &  100 & 3.798E+13 &  $\pm$ &0.48\% & 3.739E+13 &  $\pm$ &0.26\% &  \textbf{1.54\%} \\
      gmd5x5 &   10000 &  2 &   50 & 6.591E+00 &  $\pm$ &1.83\% & 6.149E+00 &  $\pm$ &0.01\% &  \textbf{6.70\%} \\
      gmd8x8 &   25600 &  2 &  128 & 5.688E+00 &  $\pm$ &1.31\% & 5.231E+00 &  $\pm$ &0.02\% &  \textbf{8.04\%} \\
       noise &   13664 &  2 &  100 & 1.095E+01 &  $\pm$ &0.89\% & 1.061E+01 &  $\pm$ &0.15\% &  \textbf{3.07\%} \\
  vardensity &   30000 &  2 &  100 & 2.624E+01 &  $\pm$ &0.43\% & 2.590E+01 &  $\pm$ &0.25\% &  \textbf{1.28\%} \\
     uniform &    1000 &  2 &  100 & 1.259E+00 &  $\pm$ &0.89\% & 1.206E+00 &  $\pm$ &0.86\% &  \textbf{4.21\%} \\
   sq6x6-2x2 &    3600 &  2 &  144 & 2.193E+00 &  $\pm$ &1.09\% & 2.041E+00 &  $\pm$ &0.00\% &  \textbf{6.94\%} \\
  randangles &    3840 &  2 &   60 & 3.456E+00 &  $\pm$ &1.83\% & 3.272E+00 &  $\pm$ &0.00\% &  \textbf{5.30\%} \\
      stains &   10000 &  2 &  100 & 5.543E+05 &  $\pm$ &0.71\% & 5.399E+05 &  $\pm$ &0.26\% &  \textbf{2.60\%} \\
  correlated &    6000 &  2 &  100 & 5.638E+05 &  $\pm$ &0.59\% & 5.517E+05 &  $\pm$ &0.48\% &  \textbf{2.14\%} \\
        rice &   10000 &  2 &  120 & 2.706E+05 &  $\pm$ &1.39\% & 2.568E+05 &  $\pm$ &0.59\% &  \textbf{5.08\%} \\
\midrule
     Average &       0 &  0 &    0 & 0.000E+00 &  $\pm$ &0.00\% & 0.000E+00 &  $\pm$ &0.00\% &  \textbf{4.27\%} \\
\bottomrule
\end{tabular}
